When One Modality Rules Them All: Backdoor Modality Collapse in Multimodal Diffusion Models

While diffusion models have revolutionized visual content generation, their rapid adoption has underscored the critical need to investigate vulnerabilities, e.g., to backdoor attacks. In multimodal diffusion models, it is natural to expect that attacking multiple modalities simultaneously (e.g., text and image) would yield complementary effects and strengthen the overall backdoor. In this paper, we challenge this assumption by investigating the phenomenon of Backdoor Modality Collapse, a scenario where the backdoor mechanism degenerates to rely predominantly on a subset of modalities, rendering others redundant. To rigorously quantify this behavior, we introduce two novel metrics: Trigger Modality Attribution (TMA) and Cross-Trigger Interaction (CTI). Through extensive experiments across diverse training configurations in multimodal conditional diffusion, we consistently observe a ``winner-takes-all'' dynamic in backdoor behavior. Our results reveal that (1) attacks often collapse into subset-modality dominance, and (2) cross-modal interaction is negligible or even negative, contradicting the intuition of synergistic vulnerability. These findings highlight a critical blind spot in current assessments, suggesting that high attack success rates often mask a fundamental reliance on a subset of modalities. This establishes a principled foundation for mechanistic analysis and future defense development.

==> tabs_figs/results.tex <==
% ICML & ICLR-W Switch
% \begin{table*}[t] % ICLR-W
\begin{table*}[!ht] % ICML
\centering
\setlength{\tabcolsep}{30pt}
\caption{\textbf{Trigger Modality Attribution (TMA) and Cross-Trigger Interaction (CTI)} under three multimodal trigger pairs, two poisoning protocols (OR/AND), and three poisoning ratios.}
\renewcommand{\arraystretch}{1.0}
\resizebox{0.98\linewidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\multirow{2}{*}{\textbf{Trigger Pair}} &
\multirow{2}{*}{\textbf{Protocol}} &
\multirow{2}{*}{\textbf{Poison \%}} &
\multicolumn{3}{c}{\textbf{Evaluation Scores on $\mathcal{D}_{\mathrm{val}}$}} \\
\cmidrule(lr){4-6}
& & & $\overline{\phi}_{i}$ (\textbf{TMA$_i$}) & $\overline{\phi}_{t}$ (\textbf{TMA$_t$}) & $\overline{\mathcal{I}}$ (\textbf{CTI}) \\
\midrule

\multirow{6}{*}{\makecell[l]{\texttt{White-box} \\ + \texttt{mignneko}}}
& \multirow{3}{*}{OR}  & 1\%  & 0.0094 & 0.9550 & -0.0192 \\
&                      & 5\%  & 0.0060 & 0.9743 & -0.0089 \\
&                      & 10\% & 0.0340 & 0.8869 & -0.0668 \\
\cmidrule(lr){2-6}
& \multirow{3}{*}{AND} & 1\%  & 0.0052 & 0.9371 & -0.0056 \\
&                      & 5\%  & 0.0045 & 0.9532 & -0.0086 \\
&                      & 10\% & 0.0040 & 0.9747 & -0.0102 \\
\midrule

\multirow{6}{*}{\makecell[l]{\texttt{Eyeglasses} \\ + \texttt{anonymous}}}
& \multirow{3}{*}{OR}  & 1\%  & 0.1107 & 0.8329 & -0.2014 \\
&                      & 5\%  & 0.1200 & 0.7376 & -0.2174 \\
&                      & 10\% & 0.1404 & 0.7469 & -0.1459 \\
\cmidrule(lr){2-6}
& \multirow{3}{*}{AND} & 1\%  & 0.0932 & 0.8533 & -0.1824 \\
&                      & 5\%  & 0.1063 & 0.8907 & -0.2185 \\
&                      & 10\% & 0.1065 & 0.8947 & -0.2149 \\
\midrule

\multirow{6}{*}{\makecell[l]{\texttt{Stop-sign} \\ + \texttt{latte coffee}}}
& \multirow{3}{*}{OR}  & 1\%  & 0.0041 & 0.9687 & -0.0114 \\
&                      & 5\%  & 0.0043 & 0.9280 & -0.0094 \\
&                      & 10\% & 0.0053 & 0.9580 & -0.0109 \\
\cmidrule(lr){2-6}
& \multirow{3}{*}{AND} & 1\%  & 0.0045 & 0.9830 & -0.0093 \\
&                      & 5\%  & 0.0048 & 1.0033 & -0.0101 \\
&                      & 10\% & 0.0045 & 1.0036 & -0.0099 \\
\bottomrule
\end{tabular}
}
\label{tab:tma_cti_main}
\end{table*}

==> tabs_figs/small_tab.tex <==
% ICML & ICLR-W Switch
\begin{table}[t] % ICML
% \begin{wraptable}  % ICLR-W
    % {r}{0.55\linewidth} % ICLR-W
    % \vspace{-10pt}
    \centering
    % \small  % ICLR-W
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.05}
    \caption{ \textbf{Single-modality trigger validity.}
    % Each unimodal trigger is effective on triggered test samples, while rarely activating on clean ones.
    Trigger-pair abbreviations: \texttt{WB}+\texttt{MN} (White-box + mignneko),
    \texttt{EG}+\texttt{AN} (Eyeglasses + anonymous), and \texttt{SS}+\texttt{LC} (Stop-sign
    + latte coffee). }
    \begin{tabular}{llcc}
        \toprule \textbf{Trigger pair}                    & \textbf{Training poison} & \textbf{ASR$_{\text{clean}}$} $\downarrow$ & \textbf{ASR$_{\text{trig}}$} $\uparrow$ \\
        \midrule \multirow{2}{*}{\texttt{WB}+\texttt{MN}} & Image-only               & 0.018                                        & 0.776                                     \\
                                                          & Text-only                & 0.000                                        & 0.996                                     \\
        % \addlinespace[2pt]
        \hline
        \multirow{2}{*}{\texttt{EG}+\texttt{AN}}          & Image-only               & 0.036                                        & 0.609                                     \\
                                                          & Text-only                & 0.000                                        & 0.996                                     \\
        % \addlinespace[2pt]
        \hline
        \multirow{2}{*}{\texttt{SS}+\texttt{LC}}          & Image-only               & 0.001                                        & 0.698                                     \\
                                                          & Text-only                & 0.000                                        & 0.996                                     \\
        \bottomrule
    \end{tabular}
    \label{tab_it_only}
    % \vspace{5pt}
\end{table} % ICML
% \end{wraptable} % ICLR-W

==> tex_writing_w/4_our_metric.tex <==
\section{Diagnosing Backdoor Modality Collapse via Attribution and Interaction}
\label{sec:shapley_modality}

Our objective is to quantify how each modality contributes to backdoor activation in multimodal diffusion models, and whether the attack effect primarily stems from a subset of modalities or from genuine cross-modal interaction.
In particular, we aim to diagnose \emph{backdoor modality collapse}, where the backdoor success is dominated by triggers from a single modality while triggers in other modalities become largely ineffectual.
We propose two new metrics, namely \textit{Trigger Modality Attribution (TMA)} and \textit{Cross-Trigger Interaction (CTI)}, to capture per-modality trigger contributions and their non-additive interaction effects, respectively.
%Next, we detail our evaluation metrics.

\paragraph{Setup (general multi-modality intervention).}
Consider an $M$-modal input $x=(x^{(1)},x^{(2)},\dots,x^{(M)})$ with modality set
$\mathcal{M}\triangleq\{1,2,\dots,M\}$.
We treat modalities as \emph{players} in an $M$-player cooperative game.
For any coalition $S\subseteq\mathcal{M}$, we define an intervention operator $\mathcal{G}_{S}$ that
\emph{activates} the trigger only on modalities in $S$ while keeping modalities in $\mathcal{M}\setminus S$ clean:
\begin{equation}
\tilde{x}_{S} \triangleq \mathcal{G}_{S}(x),
\qquad S\subseteq\mathcal{M}.
\label{eq:coalition_input_general}
\end{equation}

\paragraph{Per-example value function.}
For each example $x$ under coalition $S$, the model produces a \emph{trigger score}
$\mathrm{score}^{\mathrm{tr}}_{x}(S)$ and a \emph{normal score} $\mathrm{score}^{\mathrm{nr}}_{x}(S)$.
We define the score as
\begin{equation}
\Delta_x(S)
~\triangleq~
\mathrm{score}^{\mathrm{tr}}_{x}(S)-\mathrm{score}^{\mathrm{nr}}_{x}(S).
\label{eq:margin_general}
\end{equation}
% Since $v_x(S)$ is computed from deterministic model scores, we evaluate each coalition without Monte-Carlo estimation.
In our implementation, both $\mathrm{score}^{\mathrm{tr}}_{x}(S)$ and $\mathrm{score}^{\mathrm{nr}}_{x}(S)$
are defined based on the cosine similarity in the CLIP~\cite{clip} embedding space.
Specifically, let $\hat{y}_{x}(S)$ denote the visual output generated by the model given the coalition input
$\tilde{x}_S$, and let $y^{\mathrm{tr}}$ and $y^{\mathrm{cl}}$ denote the target (backdoor) output and the clean
reference output, respectively.
We use a pretrained CLIP image encoder $E_{\mathrm{CLIP}}(\cdot)$ to map an image into a feature vector.
Then we define
\begin{equation}
\mathrm{score}^{\mathrm{tr}}_{x}(S)
~=~
\cos\!\Big(
E_{\mathrm{CLIP}}\!\big(\hat{y}_{x}(S)\big),
E_{\mathrm{CLIP}}\!\big(y^{\mathrm{tr}}\big)
\Big),
\label{eq:trigger_score_clip}
\end{equation}
and
\begin{equation}
\mathrm{score}^{\mathrm{nr}}_{x}(S)
~=~
\cos\!\Big(
E_{\mathrm{CLIP}}\!\big(\hat{y}_{x}(S)\big),
E_{\mathrm{CLIP}}\!\big(y^{\mathrm{cl}}\big)
\Big),
\label{eq:normal_score_clip}
\end{equation}
where $\cos(\mathbf{a},\mathbf{b})=\frac{\mathbf{a}^{\top}\mathbf{b}}{\|\mathbf{a}\|_2\,\|\mathbf{b}\|_2}$
denotes cosine similarity.
Accordingly, the per-example value function $\Delta_x(S)$ in Eq.~\eqref{eq:margin_general}
measures whether the generated output is closer to the backdoor target than to the clean reference under coalition $S$.


\paragraph{Per-example attack Shapley attribution.}
Given the cooperative game $(v_x,\mathcal{M})$, the Shapley value (SV)~\cite{shapley1953value} assigns each modality
its \emph{expected marginal contribution} for example $x$:
% ICML & ICLR-W Switch
\begin{equation}
\phi^{\mathrm{mod}}_{x,m}
~=~
\sum_{S\subseteq \mathcal{M}\setminus\{m\}}
\frac{|S|!\,(M-|S|-1)!}{M!}
\Big(v_x(S\cup\{m\}) - v_x(S)\Big),
\qquad m\in\mathcal{M}.
\label{eq:shapley_general_m}
\end{equation}

% \begin{multline}
% \label{eq:shapley_general_m}
% \phi^{\mathrm{mod}}_{x,m}
% =
% \sum_{\mathclap{S\subseteq \mathcal{M}\setminus\{m\}}}
% \frac{|S|!(M-|S|-1)!}{M!}
% \big(v_x(S\cup\{m\}) - v_x(S)\big), \\
% \quad m\in\mathcal{M}.
% \end{multline} % ICML
\textit{A higher value} indicates that this modality’s trigger contributes more to backdoor success, implying \textit{a stronger trigger modality}, and vice versa.
By the efficiency axiom of SV, the total backdoor lift decomposes as
\begin{equation}
\sum_{m\in\mathcal{M}}\phi^{\mathrm{mod}}_{x,m}
~=~
v_x(\mathcal{M})-v_x(\emptyset).
\label{eq:efficiency_general_m}
\end{equation}

\paragraph{Cross-modal synergy (interaction beyond additivity).}
While the SV provides a principled semivalue to distribute the overall worth to individual entities, it does not reveal synergies or redundancies between entities; Shapley interactions extend SV by assigning joint contributions to groups 
and thereby address this limitation 
\cite{shapiq}.
In our multi-modality backdoor game, we define the \emph{total synergy} of example $x$ as the gap between the joint-coalition payoff and the sum of unimodal payoffs:
\begin{equation}
\mathrm{Syn}_{x}
~\triangleq~
v_x(\mathcal{M})
-\sum_{m\in\mathcal{M}}v_x(\{m\})
+(M-1)\,v_x(\emptyset).
\label{eq:synergy_general_m}
\end{equation}
$\mathrm{Syn}_x>0$ indicates super-additive cooperation across modalities, while $\mathrm{Syn}_x<0$ suggests interference.
% Reporting $\mathrm{Syn}_{x}$ alongside per-modality SV ($\phi^{\mathrm{mod}}_{x,m}$) prevents misinterpretation caused by SV's implicit redistribution of interaction effects into individual attributions, enabling a clearer diagnosis of \emph{backdoor modality collapse} versus genuinely complementary multi-trigger behavior.
Reporting $\mathrm{Syn}_{x}$ alongside per-modality SV ($\phi^{\mathrm{mod}}_{x,m}$) helps avoid confusion, since SV implicitly redistributes interaction effects into individual attributions. 
This makes it easier to distinguish \emph{backdoor modality collapse} from truly complementary multi-trigger behavior.


\paragraph{Dataset-level aggregation.}
Finally, we aggregate per-example modality attributions and cross-trigger interaction over the validation set $\mathcal{D}_{\mathrm{val}}$:
% ICML & ICLR-W Switch
\begin{equation}
\overline{\phi}_{m}
~=~
\frac{1}{|\mathcal{D}_{\mathrm{val}}|}
\sum_{x\in\mathcal{D}_{\mathrm{val}}}\phi^{\mathrm{mod}}_{x,m},
\quad % ICML
\qquad
\overline{\mathrm{Syn}}
~=~
\frac{1}{|\mathcal{D}_{\mathrm{val}}|}
\sum_{x\in\mathcal{D}_{\mathrm{val}}}\mathrm{Syn}_{x}.
\label{eq:dataset_level_general_m}
\end{equation}
Here, $\overline{\phi}_{m}$ is our \textit{Trigger Modality Attribution (TMA)} for modality $m$, measuring how much the backdoor activation is attributable to triggers from that modality on average.
Likewise, $\overline{\mathrm{Syn}}$ corresponds to our \textit{Cross-Trigger Interaction (CTI)}, capturing whether multimodal triggers exhibit complementary synergy ($\overline{\mathrm{Syn}}>0$) or redundancy/interference ($\overline{\mathrm{Syn}}<0$) at the dataset level.

Taken together, TMA and CTI provide a principled diagnosis of \emph{backdoor modality collapse} in multimodal diffusion backdoors.
They numerically characterize attacks that are primarily driven by a single modality’s trigger, while also quantifying the extent to which the backdoor genuinely relies on cross-modal coordination, thereby enabling more faithful evaluation and deeper mechanistic analysis.

% \paragraph{Interpretation.}
% Eqs.~\eqref{eq:shapley_general_m}--\eqref{eq:synergy_general_m} provide a per-example decomposition of backdoor efficacy into
% (i) modality-wise contributions $\{\phi^{\mathrm{mod}}_{x,m}\}_{m=1}^{M}$ and
% (ii) an interaction term $\mathrm{Syn}_x$ capturing cross-modal cooperation beyond additivity.
% This enables fine-grained diagnosis of dominant/weak modalities and modality interaction patterns in multimodal diffusion backdoors.


